Tighter Information-Theoretic Generalization Bounds from Supersamples

In this work, we present a variety of novel information-theoretic generalization bounds for learning algorithms, from the supersample setting of Steinke & Zakynthinou (2020)-the setting of the "conditional mutual information" framework. Our development exploits projecting the loss pair (obtained from a training instance and a testing instance) down to a single number and correlating loss values with a Rademacher sequence (and its shifted variants). The presented bounds include square-root bounds, fast-rate bounds, including those based on variance and sharpness, and bounds for interpolating algorithms etc. We show theoretically or empirically that these bounds are tighter than all information-theoretic bounds known to date on the same supersample setting.

==> data/plotLR.tex <==
\begin{subfigure}[t]{0.5\columnwidth}%
\centering%
\captionsetup{font=small}%
\scalebox{0.5}{
\begin{tikzpicture}
\begin{axis}
[
% legend style={at={(1,0.2)},nodes={scale=0.9, transform shape}},
% ymode=log,
legend cell align={left},
% ymode=log,
ymax=0.6,
ymin=0,
xlabel=Number of Sample ($n$),
% table/col sep=comma,
grid style=dashed,
xmin=4,
    xmax=81,
% width=5cm,
%     height=7cm,
xmajorgrids=true,
ymajorgrids=true,
ylabel=$\mathrm{Err}$.
]
\addplot[line width=2pt, color=orange] table [y=LD, x=num]{./data/LR1.txt};
\addlegendentry{LD}
\addplot[line width=2pt, color=red] table[y=SL, x=num]{./data/LR1.txt};
\addlegendentry{SL}
% \addplot[line width=2pt, color=blue] table [y=eCMI, x=num]{./data/LR1.txt};
% \addlegendentry{eCMI}
\addplot[line width=2pt, color=green] table[y=SubFast, x=num]{./data/LR1.txt};
\addlegendentry{Sub Fast}
\addplot[line width=2pt, color=cyan] table [y=VarFast, x=num]{./data/LR1.txt};
\addlegendentry{Var Fast}
\addplot[line width=2pt, color=black] table[y=Gap, x=num]{./data/LR1.txt};
\addlegendentry{Err}
\end{axis}
\end{tikzpicture}
}
\caption{Logistic Regression (Normal)}%
\label{fig:lg-normal}
\end{subfigure}%\hfill
\begin{subfigure}[t]{0.5\columnwidth}%
\centering%
\captionsetup{font=small}%
\scalebox{0.5}{
\begin{tikzpicture}
\begin{axis}
[
% legend style={at={(1,0.2)},nodes={scale=0.9, transform shape}},
% ymode=log,
legend cell align={left},
% ymode=log,
ymax=1,
ymin=0.05,
xlabel=Number of Sample ($n$),
% table/col sep=comma,
grid style=dashed,
xmin=4,
    xmax=81,
% width=5cm,
%     height=7cm,
xmajorgrids=true,
ymajorgrids=true,
ylabel=$\mathrm{Err}$.
]
\addplot[line width=2pt, color=orange] table [y=LD, x=num]{./data/LR01.txt};
\addlegendentry{LD}
\addplot[line width=2pt, color=red] table[y=SL, x=num]{./data/LR01.txt};
\addlegendentry{SL}
% \addplot[line width=2pt, color=blue] table [y=eCMI, x=num]{./data/LR01.txt};
% \addlegendentry{eCMI}
\addplot[line width=2pt, color=green] table[y=SubFast, x=num]{./data/LR01.txt};
\addlegendentry{Sub Fast}
\addplot[line width=2pt, color=cyan] table [y=VarFast, x=num]{./data/LR01.txt};
\addlegendentry{Var Fast}
\addplot[line width=2pt, color=black] table[y=Gap, x=num]{./data/LR01.txt};
\addlegendentry{Err}
\end{axis}
\end{tikzpicture}
}
\caption{Logistic Regression (Hard)}%
\label{fig:lg-hard}
\end{subfigure}%\hfill
\begin{subfigure}[t]{0.5\columnwidth}%
\centering%
\captionsetup{font=small}%
\scalebox{0.5}{
\begin{tikzpicture}
\begin{axis}
[
% legend style={at={(1,0.2)},nodes={scale=0.9, transform shape}},
% ymode=log,
legend cell align={left},
% ymode=log,
ymax=0.4,
ymin=0,
xlabel=Number of Sample ($n$),
% table/col sep=comma,
grid style=dashed,
xmin=4,
    xmax=81,
% width=5cm,
%     height=7cm,
xmajorgrids=true,
ymajorgrids=true,
ylabel=$\mathrm{Err}$.
]
\addplot[line width=2pt, color=orange] table [y=LD, x=num]{./data/LR5.txt};
\addlegendentry{LD}
\addplot[line width=2pt, color=red] table[y=SL, x=num]{./data/LR5.txt};
\addlegendentry{SL}
% \addplot[line width=2pt, color=blue] table [y=eCMI, x=num]{./data/LR01.txt};
% \addlegendentry{eCMI}
\addplot[line width=2pt, color=green] table[y=SubFast, x=num]{./data/LR5.txt};
\addlegendentry{Sub Fast}
\addplot[line width=2pt, color=cyan] table [y=VarFast, x=num]{./data/LR5.txt};
\addlegendentry{Var Fast}
\addplot[line width=2pt, color=black] table[y=Gap, x=num]{./data/LR5.txt};
\addlegendentry{Err}
\addplot[line width=2pt, color=blue] table [y=SIB, x=num]{./data/LR5.txt};
\addlegendentry{Interp.}
\end{axis}
\end{tikzpicture}
}
\caption{Logistic Regression (Interp.)}%
\label{fig:lg-easy}
\end{subfigure}%\hfill

